A Novel Quantum Augmented Framework to Improve Microgrid Cybersecurity

Small modular nuclear reactors (SMRs) are redefining the energy generation landscape by enabling the deployment of modular, scalable, and pre-built power units that can be used to build distributed autonomous microgrids for critical infrastructure and burgeoning AI factories. Often, these microgrids are linked together to provide a resilient, decentralized power generation infrastructure. Consequently, the cybersecurity of microgrids is of critical importance. In this work, we propose a quantum augmented network framework for resilient microgrids. We integrate the ideas of secure quantum networking, quantum anonymous notification, and quantum random number generation to strengthen the integrity, confidentiality, and privacy of microgrid networks. To substantiate the possible benefits of using quantum augmented microgrids, we simulate a practical high-impact classical attack: a traffic analysis and priority-action spoofing campaign that can (1) deanonymize the anonymous notification for a high-priority action, (2) force excessive key usage, and (3) induce harmful allow/block operations at the control level. We quantify how these attacks affect information leakage, spoof acceptance, key sufficiency, and operational outcomes such as latency, deadline misses, unserved energy, etc. This quantum augmented microgrid (QuAM) framework lets us evaluate trade-offs between privacy, availability, and the operational cost of mitigation (cover traffic, verification delays, and key-rotation policies), further paving the path for the study of more nuanced attacks that arise due to the use of quantum-classical integrated frameworks.

==> na.tex <==
\begin{tcolorbox}[title=Example Q-HTTP Exchange, colback=white]
\small
\textbf{Request (from Alice):}
\begin{verbatim}
Q-SEND /secure-email HTTP/1.1
Host: bob.example.com
Q-Encryption-Mode: quantum
X-Quantum-Channel-ID: 1
Content-Type: application/octet-stream

[Encrypted Email Body (using QKD-derived key)] (Assuming quantum encryption entails that)
\end{verbatim}

\textbf{Response (from Bob):}
\begin{verbatim}
HTTP/1.1 200 OK
Q-Quantum-Status: success

[Optional: Status information, key index, etc.]
\end{verbatim}
\end{tcolorbox}


\begin{figure}[ht!]
\centering
\begin{tikzpicture}[%
  node distance=1.5cm, % Adjust spacing between layers
  >=latex, 
  every node/.style={font=\small, align=center},
  xscale=1.0,
  yscale=1.0
]

% Define colors for layers
\definecolor{layer7}{HTML}{FFD700} % Gold for Layer 7
\definecolor{layer6_5}{HTML}{87CEFA} % Light blue for Layer 6-5
\definecolor{layer4}{HTML}{90EE90} % Light green for Layer 4
\definecolor{layer3}{HTML}{FFB6C1} % Light pink for Layer 3
\definecolor{layer2}{HTML}{FFA07A} % Light salmon for Layer 2
\definecolor{layer1}{HTML}{D8BFD8} % Thistle for Layer 1

%-------------------------
% Alice's Layers (Left)
%-------------------------
\node(A7) [rectangle, draw=black, fill=layer7, text width=3.5cm] 
  {\textbf{L7:}\\ Q-HTTP +\\ Privacy Classifier};

\node(A6_5) [rectangle, draw=black, fill=layer6_5, below of=A7, text width=3.5cm] 
  {\textbf{L6--5:}\\ QKD / Session};

\node(A4) [rectangle, draw=black, fill=layer4, below of=A6_5, text width=3.5cm] 
  {\textbf{L4:}\\ TCP};

\node(A3) [rectangle, draw=black, fill=layer3, below of=A4, text width=3.5cm] 
  {\textbf{L3:}\\ IP};

\node(A2) [rectangle, draw=black, fill=layer2, below of=A3, text width=3.5cm] 
  {\textbf{L2:}\\ Ethernet +\\ Quantum Signals};

\node(A1) [rectangle, draw=black, fill=layer1, below of=A2, text width=3.5cm] 
  {\textbf{L1:}\\ WDM Coupler\\($\lambda_c,\;\lambda_q$)};

% Group Alice's layers into a box labeled "Sender"
\node [draw=black, fit={(A7) (A1)}, inner sep=0.5cm, label={[anchor=north]south:Sender's End}] {};

%-------------------------
% Single Fiber (Center)
%-------------------------
\node(F) [rectangle, draw=black, 
  minimum height=9cm,
  text width=3cm, right of=A4, xshift=3cm, yshift=-0.5cm] 
  {\textbf{Optical Fiber}\\
   (WDM: $\lambda_c + \lambda_q$)};

%-------------------------
% Bob's Layers (Right)
%-------------------------
\node(B7) [rectangle, draw=black, fill=layer7, text width=3.5cm, right of=F, xshift=3cm, yshift=4.5cm] 
  {\textbf{L7:}\\ Q-HTTP Server};

\node(B6_5) [rectangle, draw=black, fill=layer6_5, below of=B7, text width=3.5cm] 
  {\textbf{L6--5:}\\ QKD / Session};

\node(B4) [rectangle, draw=black, fill=layer4, below of=B6_5, text width=3.5cm] 
  {\textbf{L4:}\\ TCP};

\node(B3) [rectangle, draw=black, fill=layer3, below of=B4, text width=3.5cm] 
  {\textbf{L3:}\\ IP};

\node(B2) [rectangle, draw=black, fill=layer2, below of=B3, text width=3.5cm] 
  {\textbf{L2:}\\ Ethernet +\\ Quantum Detection};

\node(B1) [rectangle, draw=black, fill=layer1, below of=B2, text width=3.5cm] 
  {\textbf{L1:}\\ WDM Coupler\\($\lambda_c,\;\lambda_q$)};

% Group Bob's layers into a box labeled "Receiver"
\node [draw=black, fit={(B7) (B1)}, inner sep=0.5cm, label={[anchor=north]south:Receiver's End}] {};

%-------------------------
% Arrows for Message Flow
%-------------------------

% Alice's downward flow
\draw[->] (A7.south) -- (A6_5.north);
\draw[->] (A6_5.south) -- (A4.north);
\draw[->] (A4.south) -- (A3.north);
\draw[->] (A3.south) -- (A2.north);
\draw[->] (A2.south) -- (A1.north);

% Across the fiber
\draw[->] (A1.east) -- (F.west); % From Alice's L1 to Fiber
\draw[->] (F.east) -- (B1.west); % From Fiber to Bob's L1

% Bob's upward flow
\draw[->] (B1.north) -- (B2.south);
\draw[->] (B2.north) -- (B3.south);
\draw[->] (B3.north) -- (B4.south);
\draw[->] (B4.north) -- (B6_5.south);
\draw[->] (B6_5.north) -- (B7.south);

\end{tikzpicture}
\vspace{0.2cm}
\caption{Single-Fiber Q-HTTP Architecture. Alice’s ML Privacy Classifier (L7) determines if quantum security (QKD) is required (\texttt{label=1}). Messages flow downward through Alice's layers (L7 to L1), pass through the optical network fiber (via WDM $\lambda_c + \lambda_q$), and flow upward through Bob's layers (L1 to L7). The ``Sender" and ``Receiver" groups encapsulate the respective layers.}
\label{fig:layers}
\end{figure}
